New Methods, Current Trends and Software Infrastructure for NLP

The increasing use of `new methods' in NLP, which the NeMLaP conference series exemplifies, occurs in the context of a wider shift in the nature and concerns of the discipline. This paper begins with a short review of this context and significant trends in the field. The review motivates and leads to a set of requirements for support software of general utility for NLP research and development workers. A freely-available system designed to meet these requirements is described (called GATE - a General Architecture for Text Engineering). Information Extraction (IE), in the sense defined by the Message Understanding Conferences (ARPA \cite{Arp95}), is an NLP application in which many of the new methods have found a home (Hobbs \cite{Hob93}; Jacobs ed. \cite{Jac92}). An IE system based on GATE is also available for research purposes, and this is described. Lastly we review related work.

==> references.tex <==
%auto-ignore
%
%	references.tex - GUTTER
%
%	Hamish Cunningham, 12/06/95
%
%	$Id: references.tex,v 1.1 1996/04/12 13:05:51 hamish Exp $


\section{\label{references}References}

\small

(Alshawi 1992) H. Alshawi, ed., The Core Language Engine, MIT Press,
Cambridge Mass., 1992.
\\ %
(ARPA 1992) Advanced Research Projects Agency,
{\em Proceedings of the Fourth Message Understanding Conference (MUC-4)},
Morgan Kaufmann, 1992.
\\ %
(ARPA 1993a) Advanced Research Projects Agency,
{\em Proceedings of TIPSTER Text Program (Phase I)}
Morgan Kaufmann, 1993.
\\ %
(ARPA 1993b) Advanced Research Projects Agency,
{\em Proceedings of the Fifth Message Understanding Conference (MUC-5)},
Morgan Kaufmann, 1993.
\\ %
(ARPA 1996) Advanced Research Projects Agency,
{\em Proceedings of the Sixth Message Understanding Conference (MUC-6)},
Morgan Kaufmann, 1996.
\\ %
(Ballim 1995) A. Ballim, {\em Abstract Data Types for MULTEXT Tool I/O},
LRE 62-050 Deliverable 1.2.1, 1995.
\\ %
(Bartell, Cottrell, Belew 1994) B.T. Bartell, G.W. Cottrell, R.K. Belew,
{\em Automatic Combination of Multiple Ranked Retrieval Systems},
proceedings of SIGIR 1994.
\\ %
(Beale, Nirenburg, Mahesh 1995)
S. Beale, S. Nirenburg, K. Mahesh.
{\em Semantic Analysis in
the Mikrokosmos Machine Translation Project},
{\em Proceedings of the Second Symposium on Natural Language Processing
(SNLP-95)}, August 2-4, 1995, Bangkok, Thailand.
\\ %
(Black ed. 1991) W.J. Black (ed.), {\em PLUS -- a Pragmatics-Based Language
Understanding System, Functional Design}, ESPRIT P5254 Deliverable D1.2,
1991.
\\ %
(Bod 1995) R. Bod, {\em Enriching Linguistics with Statistics: Performance
Models of Natural Language}, PhD thesis,
Institute for Logic, Language and Computation,
University of Amsterdam 1995.
\\ %
(Boguraev, Garigliano, Tait 1995), B. Boguraev, R. Garigliano, J. Tait,
editorial of {\em Journal of Natural Language Engineering, Vol. 1 Part 1},
Cambridge University Press, March 1995.
\\ %
(Boitet, Seligman 1994) C. Boitet, M. Seligman, {\em The ``Whiteboard''
Architecture: A Way to Integrate Heterogeneous Components of NLP Systems},
proceedings of COLING 1994.
\\ %
(Brill 1994) E. Brill,
{\em Some Advances in Transformation-Based Part of Speech Tagging},
proceedings of The Twelfth National Conference on Artificial Intelligence
(AAAI-94), Seattle, Washington 1994.
\\ %
(Briscoe, Carroll 1993) T. Briscoe, J. Carroll, {\em Generalized
Probabilistic LR Parsing of Natural Language (Corpora) with
Unification-Based Grammars}, 
{\em Computational Linguistics} Volume 19, Number 1, March 1993.
\\ %
(Church 1988) K. Church, {\em A stochastic parts of speech program
and noun phrase parser for unrestricted text}, {\em Second
conference on Applied NLP}, ACL 1988.
\\ %
(Church, Mercer 1993) K.W. Church, R.L. Mercer, {\em Introduction to the
Special Issue on Computational Linguistics Using Large Corpora},
{\em Computational Linguistics} Volume 19, Number 1, March 1993.
\\ %
(Crouch, Gaizauskas, Netter 1995) R. Crouch, R. Gaizauskas, and K. Netter, 
{\em Interim Report of the Study Group on Assessment and Evaluation}, Report
prepared under the auspices of the EAGLES Project for the
Language Engineering Sector, Telematics Programme.
To be published shortly.
\\ %
(Cunningham, Freeman, Black 1994)
H. Cunningham, M. Freeman, W.J. Black, {\em Software Reuse, 
Object-Orientated Frameworks and Natural Language Processing}, 
Conference on New Methods in Natural Language Processing, 
Manchester 1994.
\\ %
(EAGLES 1994) {\em Evaluation of Natural Language Processing Systems}, draft
document EAG-EWG-IR.2 of the EAGLES Project for the
Language Engineering Sector, Telematics Programme,
Fourth Framework Programme of the European Commission.
\\ %
(Evans, Kilgarriff 1995) R. Evans, A. Kilgarriff, {\em Standards 
and How to do Lexical Engineering},
{\em Proceedings of the Second Language Engineering
Convention}, London 1995.
\\ %
(Farwell, Wilks 1989) D. Farwell, Y. Wilks, {\em ULTRA -- a
multilingual machine translation system}, memoranda in Computer and
Cognitive Science, CRL Las Cruces, NM 1989.
\\ %
(Gaizauskas, Humphreys, Wakao, Cunningham, Wilks 1996),
R. Gaizauskas,
K.  Humphreys, T. Wakao, H. Cunningham, Y. Wilks
{\em LaSIE -- Description of the
Sheffield System Used for MUC-6},
in (ARPA 1996).
\\ %
(Galliers, Sparck Jones 1993) J. Galliers, K. Sparck Jones, {\em Evaluating 
Natural Language Processing Systems}, Technical Report 291, Computer
Laboratory, University of Cambridge.
\\ %
(Grishman 1995a) R. Grishman, {\em TIPSTER architecture 1.50, The Tinman
Architecture}, presentation
18/5/95, slides available at
http://www.cs.nyu.edu/tipster.
\\ %
(Grishman, 1995b)  R. Grishman,
{\em TIPSTER II Architecture
Design Document Version 1.52 (Tinman Architecture)},
TIPSTER working paper 1995, available at
http://www.cs.nyu.edu/tipster.
\\ %
(Grover et al. 1993) C. Grover, J. Carroll, T. Briscoe, The Alvey Natural
Language Tools, HCRC, University of Edinburgh.
\\ %
(Hobbs 1993) J. Hobbs, The Generic Information Extraction System, in (ARPA
1993b).
\\ %
(Jacobs ed. 1992) P.S. Jacobs, ed., {\em Intelligent Text-Based Systems,
Current Researh and Practice in Information Extraction and Retrieval},
Lawrence Erlbaum, Hillsdale NJ, 1992.
\\ %
(Jelinek 1985) F. Jelinek, Self-organising Language Modeling for Speech
Recognition, IBM Technical Disclosure Bulletin, 28, 2591-2594.
\\ %
(Kuno, Oettinger 1962) S. Kuno, A. Oettinger, {\em Multiple Path
Syntaxctic Analyzer}, {\em Information
Processing} 1962 pp 306-312 Proc. IFIP 1962, Popplewell (ed.)
Amsterdam: North Holland.
\\ %
(Leech, Garside, Atwell 1983) G. Leech, R. Garside, E. Atwell, {\em The
Automatic Grammatical Tagging of the LOB Corpus}, ICAME News 7 1983.
\\ %
(Lehrberger, Bourbeau 1988) J. Lehrberger, L. Bourbeau, Machine Translation:
linguistic characteristics of MT systems
and general methodology of evaluation. J Benjamins: Amsterdam, 1988.
\\ %
(Magerman 1994) D. Magerman, {\em Natural Language Parsing as Statistical
Pattern Recognition}, PhD thesis, Department of Computer Science, Stanford,
1994.
\\ %
(Magerman 1995) D. Magerman, {\em Statistical Decision-Tree Models for
Parsing}, proceedings of ACL 1995.
\\ %
(Nirenburg 1994) S. Nirenburg, The Workstation Substrate of the Pangloss
Project, Proceedings of the Second International Workshop on fundamental
research for The Future Generation of NLP systems (FGNLP-2), UMIST,
Manchester 1992.
\\ %
(Nirenburg, Frederking, Fawell, Wilks 1994)
S. Nirenburg, R. Frederking, D. Fawell, Y. Wilks,
{\em Two Types of Adaptive MT Environments}, proceedings of COLING 94.
\\ %
(Nyberg, Mitamura, Carbonell 1994)
G.H. Nyberg, T. Mitamura, J.G.Carbonell, {\em
Evaluation Metrics for KBMT}, proceedings of COLING 1994.
\\ %
(Palmer, Finin 1990) M. Palmer, T. Finin, {\em Workshop on the Evaluation of
Natural Language Processing Systems}, {\em Computational Linguistics}, Vol.
16, Number 3.
\\ %
(Robert, Armstrong 1995) G. Robert, S. Armstrong, {\em Tagging Tool},
LRE 62-050 Deliverable 2.4.1, 1995.
\\ %
(Salton 1989) G. Salton, Automatic Text Processing: 
The Transformation, Analysis, and Retrieval of Information by Computer,
Addison-Wesley, Reading MA, 1989.
\\ %
(Simpkins, Groenendijk 1994) The ALEP Project, Cray Systems / CEC, Luxemburg
1994.
\\ %
(Sparck Jones 1994) K. Sparck Jones, {\em Towards better NLP System
Evaluation}, Proceedings 2nd ARPA Workshop on Human Language Technology.
\\ %
(Sperberg-McQueen, Burnard 1994)
Sperberg-McQueen C.M., L. Burnard, Guidelines for Electronic Text Encoding
and Interchange (TEI P3), ACH, ACL, ALLC, 1994.
\\ %
(Strzalkowski, Scheyen 1993) T. Strzalkowski, P.G.N. Scheyen, {\em
Evaluation of TTP Parser: A Preliminary Report}, PROTEUS Project Memorandum
\#58, Dept. Computer Science, New York University 1993.
\\ %
(Thompson 1995a) H. Thompson, {\em Priority On-Ramp or Squashed Hedgehog?},
invited talk, {\em Second Language Engineering Conference}, London 1995.
\\ %
(Thompson 1995b) H. Thompson, {\em MULTEXT Workpackage 2 Milestone B
Deliverable Overview}, LRE 62-050 Deliverable 2, 1995.
\\ %
(TIPSTER 1994) TIPSTER Architecture Committee, {\em TIPSTER Text Phase II
Architecture Concept}, 
TIPSTER working paper 1994, available at
http://www.cs.nyu.edu/tipster.
\\ %
(Wakao, Gaizauskas, 1995), T. Wakao, R. Gaizauskas,
{\em Evaluation of Algorithms for the Recoginition and Classification
of Proper Names}, {\em submitted}.
\\ %
(Wilks 1994) Y. Wilks, {\em Developments in MT Research in the US}, ASLIB
Proceedings, Vol. 46 \#4, April 1994.
\\ %
(Wilks, Guthrie, Guthrie, Cowie 1992)
Y. Wilks, L. Guthrie, J. Guthrie, J. Cowie, {\em
Combining Weak Methods in Large-Scale Text Processing}, in (Jacobs ed.
1992).
\\ %
(Wilks, Guthrie, Slator 1996) Y. Wilks, L. Guthrie, B. Slator, {\em Electric
Words}, MIT Press, Cambridge, MA 1996.
\\ %
(Winograd 1972) T. Winograd, {\em Understanding Natural Language}, Academic
Press, New York 1972.




% $Log: references.tex,v $
% Revision 1.1  1996/04/12  13:05:51  hamish
% as sent to Oflazer
%

